Automatically Finding Optimal Index Structure

Existing learned indexes (e.g., RMI, ALEX, PGM) optimize the internal regressor of each node, not the overall structure such as index height, the size of each layer, etc. In this paper, we share our recent findings that we can achieve significantly faster lookup speed by optimizing the structure as well as internal regressors. Specifically, our approach (called AirIndex) expresses the end-to-end lookup time as a novel objective function, and searches for optimal design decisions using a purpose-built optimizer. In our experiments with state-of-the-art methods, AirIndex achieves 3.3x-7.7x faster lookup for the data stored on local SSD, and 1.4x-3.0x faster lookup for the data on Azure Cloud Storage.

==> figures/corpus.tex <==

\begin{table}[tbp]
         \caption{Dataset Statistics. (i) \# entries: the total number of key-value pairs. (ii) Size on disk: the file size of the dataset. (iii) Key size: the fixed size of each key in bytes. (iv) Value size: the mean and standard deviation over all values.}
    \label{table:stats_table}
    % \scriptsize
    \setlength\tabcolsep{0pt}
    \begin{tabular*}{\columnwidth}{l l l l l}
    \toprule
    \multirow{2.4}{*}{\makecell{\textbf{\# entries}}} 
        & {\multirow{2.4}{*}{\makecell{\textbf{Size on disk}}}}
            & {\multirow{2.4}{*}{\makecell{\textbf{Key Size}}}}
                & \multicolumn{2}{c}{\textbf{Value Size}} \\
    % \cmidrule{3-4} 
    \cmidrule{4-5}
        &  &  & {mean} & {stddev} \\ 
    \midrule
    % {49,975,544} & {17} & {16} & {332} & {~323,675} \\
    {49,975,544} & {17 GB} & {16 bytes} & {332 bytes} & {323,675 bytes} \\
    \bottomrule
    \end{tabular*}
\end{table}


% key avg: 8.779790971359002
% key stddev: 0.4702377935811465
% value avg: 315.69970124846526
% value stddev: 196523.4624928337
% file size: 16266014686 (16GB)


==> related.tex <==
\section{Related Work}


% \todo{Goal: Appreciate other researchers (the later the better) while clarifying that
% our work is significantly *different* from theirs.
% MIT, Brown, CMU, Germany?
% Prefer conference papers to journals}

\paragraph{Learning for DBMS}

Verdict~\cite{park2017database}, IDEA~\cite{galakatos2017revisiting}, SageDB~\cite{kraska2019sagedb} and Qtune~\cite{li2019qtune} \toreview{exploit} the answers to past queries for more accurate approximate query processing. BlinkML~\cite{park2019blinkml} uses sampling to reduce time and computational costs for machine learning models that are based on maximum likelihood estimations. QuickSel~\cite{park2020quicksel} and Naru~\cite{naru2019} \toreview{produce} more accurate selectivity estimates using models that learn from queries. Leo~\cite{markl2003leo}, Neo~\cite{marcus2019neo} and Bao~\cite{marcus2021bao} are query optimizers that learn from past queries to improve query execution planning. However, all databases above are based on local storage and \toreview{focus} more on the query plan optimization while \system \toreview{places} more emphasis on the learned index for cloud storage.

% Verdict \cite{park2017database} is a query engine based on the observation that database performance can be improved by learning from past query answers and exploiting the knowledge to answer queries more analytically.
% yongjoo: quicksel: learning-based selectivity estimation
% yongjoo: blinkml: sampling-based machine learning
% Deep Unsupervised Cardinality Estimation: Deep learning-based cardinality estimation
% Tim Kraska: https://dblp.org/pid/26/6037.html
% \todo{Good place to self-cite Yongjoo's work}


\paragraph{Learning Indexes}

Kraska et al.~\cite{kraska2018case} proposed that indexes can be built using traditional ML techniques by learning the cumulative distribution function of the input data, with the observation that indexes can be thought of as models. ALEX \cite{ding2020alex}, SIndex~\cite{wang2020sindex},\toreview{and} XIndex \cite{tang2020xindex} built upon this idea and introduced support for additional types of workload that were originally not supported in \cite{kraska2018case}. \system is different in that it is designed specifically for cloud storage, while existing learning-based index structures are all optimized for in-memory or local disk storage, which allows us to achieve low cold state end to end latency.


\paragraph{Other Index Structures}

B-tree~\cite{bayer1972organization} is a common index structure in database systems due to its efficiency, self-balancing, and cheap reorganization~\cite{comer1979ubiquitous}. There has been substantial work in running B-tree index in cloud and distributed settings ~\cite{wu2010efficient, sowell2012minuet}. LSM-tree is another index structure that is widely adopted in systems like BigTable~\cite{chang2008bigtable}, LevelDB~\cite{leveldb}, RocksDB~\cite{rocksdb}\toreview{,} and AsterixDB~\cite{altwaijry2014asterixdb} for its high space efficiency and low write amplification. Apache Lucene~\cite{lucene} is a library \toreview{that provides} indexing and searching capabilities using an inverted index built on the skip-list~\cite{pugh1990skip} data structure. Apache Lucene is widely used in systems like ElasticSearch~\cite{elasticsearch} and Apache Solr~\cite{solr}.

% \todo{See our literature review on distributed B-trees or so. RocksDB, LevelDB, Elasearch, Apache Lucence, che Solr}
\todo{Although all} Learning-based Index Structures and other conventional indexes are well-designed and demonstrate great performance under \toreview{fast storage environments}(such as SSD, NVMe, memory, L1 cache, etc.). They were not originally designed for cloud storage. Admittedly, some of them may achieve good results on cloud storage when the system has been running for a long time \toreview{and the index structures and data have mostly been cached}. However, if the system is in the cold state or \toreview{the dataset} is too large for the memory, most of them would \toreview{encounter bottlenecks to due inherent local storage assumptions in their design}.


\paragraph{Database Systems in the Cloud-era} 

Cloud storage has become an attractive tier of storage for database systems due to its cost efficiency, low latency, and high durability. There is substantial research \toreview{delicated to running} a SQL query engine directly against cloud storage. Presto~\cite{sethi2019presto} is a distributed SQL query engine for large scale datasets stored either on-premise or in cloud environments. Redshift Spectrum~\cite{redshiftspectrum21} is a scalable and multi-tenant processing layer of Amazon Redshift that provides integrated access to relational tables in the database and objects in open-file formats such as Amazon S3. Snowflake~\cite{dageville2016snowflake} provides a multi-tenant, transactional, secure, highly scalable, and elastic data warehouse as a service in the cloud. Lakehouse~\cite{armbrust2021lakehouse} is a unified data platform based on Apache Spark~\cite{spark2012} that implements data warehousing functionality over open file
formats for \toreview{a} data lake in the cloud.

Cloud function services that provide serverless code execution functionality have started to gain research interest as an alternative to provisioned compute clusters, due to the bursty and low volume nature of analytic workloads. Starling~\cite{perron2020starling} and Lambdada~\cite{muller2020lambada} are examples of data analytics systems built on cloud function services. Compared to provisioned compute clusters, the use of serverless platforms for data analytics can achieve lower \toreview{costs and operation burdens} with competitive query performance.

% Elasticity is an important aspect of large scale systems because it allows for cost reduction and performance improvement. There has been increasing amount of research into supporting elasticity for various types of applications. Dynamo \cite{sivasubramanian2012amazon}, Accordion \cite{serafini2014accordion} and NashDB \cite{marcus2018nashdb} are examples of elastic DBMS, while Snowflake \cite{dageville2016snowflake} and Lakehouse \cite{armbrust2021lakehouse} support elastic data warehousing and analytics. Elasticity of machine learning algorithms have also been an active area of research in recent years~\cite{liberty2020elastic,xiao2018gandiva}. Elasticity is an important property of \system. In particular, it is automatically scalable based on workload without any operator intervention.



% \todo{SoCC, OOPSLA, NSDI(?), SOSP, OSDI, VLDB, SIGMOD, CIDR(?)}
